Alternating minimization for dictionary learning: Local Convergence Guarantees

We present theoretical guarantees for an alternating minimization algorithm for the dictionary learning/sparse coding problem. The dictionary learning problem is to factorize vector samples $y^{1},y^{2},\ldots, y^{n}$ into an appropriate basis (dictionary) $A^*$ and sparse vectors $x^{1*},\ldots,x^{n*}$. Our algorithm is a simple alternating minimization procedure that switches between $\ell_1$ minimization and gradient descent in alternate steps. Dictionary learning and specifically alternating minimization algorithms for dictionary learning are well studied both theoretically and empirically. However, in contrast to previous theoretical analyses for this problem, we replace a condition on the operator norm (that is, the largest magnitude singular value) of the true underlying dictionary $A^*$ with a condition on the matrix infinity norm (that is, the largest magnitude term). Our guarantees are under a reasonable generative model that allows for dictionaries with growing operator norms, and can handle an arbitrary level of overcompleteness, while having sparsity that is information theoretically optimal. We also establish upper bounds on the sample complexity of our algorithm.

==> acknowledgments.tex <==
We gratefully acknowledge the support of the NSF through grant
IIS-1619362, and of the Australian
Research Council through an Australian Laureate Fellowship
(FL110100281) and through
the ARC Centre of Excellence for Mathematical and Statistical
Frontiers. Thanks also to the Simons
Institute for the Theory of Computing Spring 2017 Program on
Foundations of Machine Learning. The authors would like to thank Sahand Negahban for pointing out an error in the $\mu$-incoherence assumption in an earlier version. 


==> finite.tex <==
(\emph{To add: Uniform law of large numbers by Mcdiarmid's inequality. The finite sample guarantees follow from a standard application of Bernstein's inequality for sparse random variables. Following this application we end up with a sample complexity of $n = \tilde{\Omega}(r)$, which is better than the previous sample complexity results for the dictionary learning setting.)}

==> lb_bell.tex <==
(\emph{To add: This lower bound follows from similar Fano's bound argument presented in ``{\it Linear and Conic Programming Estimators in High-dimensional Errors-in variables Models -- Alexandre Belloni, Mathieu Rosenbaum and Alexandre B. Tsybakov}."})

%To derive the lower bounds we apply Theorem 2.7 in [Tsybayakov Nonparametric estimation.]. We define a finite set of ``hypotheses" included in $\mathbb{B}_0(s) \cap S_2(R)$. To this end, we first introduce
%
%\begin{align*}
%\mathcal{M} = \{ x \in \{0,1\}^{p-1}: \rho_H(0,x) = s-1\}
%\end{align*}
%
%where $\rho_H$ denotes the Hamming distance between elements of $\{0,1 \}^{p-1}$, and $\boldsymbol{0}$ is the zero vector. Then, there exists a subset $\mathcal{M}'$ of $\mathcal{M}$ such tat for any $x,x' \in \mathcal{M}'$ with $x \neq x'$, we have $\rho_H(x,x') > s/16$ and also 
%
%\begin{align}
%\log \lvert \mathcal{M}'\rvert \ge c_1 s \log\big(\frac{r}{s}\big)
%\end{align}
